GPT Struct Me: Probing GPT Models on Narrative Entity Extraction

The importance of systems that can extract structured information from textual data becomes increasingly pronounced given the ever-increasing volume of text produced on a daily basis. Having a system that can effectively extract such information in an interoperable manner would be an asset for several domains, be it finance, health, or legal. Recent developments in natural language processing led to the production of powerful language models that can, to some degree, mimic human intelligence. Such effectiveness raises a pertinent question: Can these models be leveraged for the extraction of structured information? In this work, we address this question by evaluating the capabilities of two state-of-the-art language models -- GPT-3 and GPT-3.5, commonly known as ChatGPT -- in the extraction of narrative entities, namely events, participants, and temporal expressions. This study is conducted on the Text2Story Lusa dataset, a collection of 119 Portuguese news articles whose annotation framework includes a set of entity structures along with several tags and attribute values. We first select the best prompt template through an ablation study over prompt components that provide varying degrees of information on a subset of documents of the dataset. Subsequently, we use the best templates to evaluate the effectiveness of the models on the remaining documents. The results obtained indicate that GPT models are competitive with out-of-the-box baseline systems, presenting an all-in-one alternative for practitioners with limited resources. By studying the strengths and limitations of these models in the context of information extraction, we offer insights that can guide future improvements and avenues to explore in this field.

==> scratch.tex <==
When choosing what models to employ on our research  several level had to be taken into account.

Effectiveness. We wanted the models in the study to be be able to attain state-of-the-art effectiveness on the tasks. To guarantee that our research in

Hardware requirements. The most effective language models are (most often) the ones with the largest set of parameters. For instances, on the LLaMA models, the model with $65$ billion parameters is more effective than the one with $7$ billion~\cite{Touvron2023LLaMA:Models}. In order to do inference with this systems one requeris specific hardaware capable of executing the predictions of this models, which is not with access of have access.

Availability. Although several large language models have been produced with the research papers being published, most of them are not released or available to the general public\footnote{\url{https://github.com/Mooler0410/LLMsPracticalGuide}}. Examples of this are the PaLM~\cite{Chowdhery2022PaLM:Pathways} and Chinchilla~\cite{Hoffmann2022TrainingModels} models.

Domain. The models in the study should be for general domain, not tuned to a specific task, as is the case of CodeX~\cite{Chen2021EvaluatingCode}, which was optimized to produce code, and Galatica~\cite{Taylor2022Galactica:Science}, which was optimized for scientific texts.

When taken all this factors into account GPT-3 and GPT-3.5, most commonly known as ChatGPT, became the obvious choice. 



% Interpreting a narrative requires two main levels of information. The first is the identification of the entities that take part in it. An the second is to relate those entities. By correctly completing these two layers one can produce a structured representation of the narrative and store it in a database which then can be queried in a programmatic manner, allowing it to be used in different applications. This work focuses in accessing if state-of-the-art language models are able to attain the first level of information.

% This domain is characterized by two main levels of information. The first is the identification of the entities that take part in the narrative. The second is to relate those entities. By correctly completing these two layers one can produce a structured representation of the narrative and store it in a database which then can be queried in a programmatic manner, allowing it to be used in different applications~\cite{Santana2023AData}. 

% Our work evaluates the capabilities of large language models on the first step in the extraction of structured information from a narrative. This step comprises the identification of the tokens that refer to entities within the narrative context. Typically, the most frequent entities in this regard are events, participants, and timexs. 

Furthermore, given that there is still a limited number of NLP tools for European Portuguese, a good effectiveness of pre-trained LLMs in this language and task can lead to new and interesting research paths in this domain. 

However, since LLMs are trained using selected text data from the Internet, their effectiveness is impacted by the language in which the data is more persistent. Therefore, NLP research conducted in low-resource languages is still a challenging task~\cite{Magueresse2020Low-resourceChallenges}. Although recent LLMs are pushing the effectiveness of NLP tasks in these languages, it is not clear yet what is the effectiveness of these LLMs in less traditional and more complex NLP tasks.


To be more specific, we do an ablation study over three levels of information to include in the prompt: the (general) entity definition as it was provided to the annotator on the annotation process; one example of document with the annotation; a rather then just to exrtract soly the entities we also ask the model to classify their class


acess the model capabilities of  with different levels of information by doing an albation study different prompt templates on a subset of $20$ documents of the dataset.   This different levels  we perform an ablation study on a subset of $20$ the news articles to select the best prompt template for each entity, model pair. Then, we use the best prompt templates to evaluate the models effectiveness on the remaining documents of the corpus. 

These include a detailed definition of the task objective, the definition of each of the entities we want to extract, and a one-shot example document that provides the input along with the target output on the prompt. 

 However, each time an example is passed down in the prompt, the model is fed a clear annotation of the expected output, which is likely to improve the effectiveness of the results due to the specificity of the tasks being evaluated. Therefore, for a better characterization of the capabilities of GPT-3 and ChatGPT, we will consider the best prompts for both cases. 


%To evaluate the models, we conducted a series of experiments using various prompt templates on a subset of $20$ carefully sampled documents. These documents were selected to be representative of the entire dataset, ensuring that the resulting statistics from this study provide a reliable estimate of the overall effectiveness of the prompt template. The experimentation involved an ablation study where we examined three components that make up the prompt template. We identified the best prompt templates for each entity-model pair and use them to assess the model's effectiveness on the remaining documents in the dataset. These values are then compared with out-of-the-box baseline systems to assess if the GPT models can be considered a reliable approach. By employing this methodology, we aimed to thoroughly probe the capabilities of the model and gather valuable insights into its effectiveness.

Tools that can automatically extract the narrative structure from textual data are becoming increasingly important given the ever-increasing volume of complex text produced. Several domains, such as finance, health, justice, and media would benefit from the ability to seamlessly obtain the narrative elements in documents. Recent developments in natural language processing led to the production of powerful language models that can efficiently produce very useful output given non formal prompts. Such effectiveness raises a pertinent question: Can these models be leveraged for the extraction of structured information? In this paper, we address this question by evaluating the answers to different prompts of two state-of-the-art language models -- GPT-3 and GPT-3.5, commonly known as ChatGPT -- for the extraction of narrative entities, namely events, participants, and temporal expressions. This study is conducted on the Text2Story Lusa dataset, a collection of 119 news articles densely annotated under a semantic narrative framework. It is important to note that the dataset was only publicly released after the development of this research. This ensures that the annotated corpus was not part of the data used to train these models, enabling a fair assessment of their effectiveness. For the evaluation of the models' response, we first select the best prompt template through an ablation study over prompt components that provide varying degrees of information on a subset of documents of the dataset. Subsequently, we use the best templates to evaluate the effectiveness of the models on the remaining documents. The results obtained indicate that GPT models, although not clearly superior, are competitive with out-of-the-box baseline systems, presenting an all-in-one alternative for practitioners with limited resources. By studying the strengths and limitations of these models in the context of information extraction, we offer insights that can guide future improvements and avenues to explore in the field of information extraction by prompting, with a focus on narrative extraction. 

==> tables/data.tex <==
\begin{table*}[ht]
\caption{Definitions, class types, count, and examples of events, participants, and timexs in the Text2Story Lusa Dataset.}\label{tab:data}
\centering
\begin{tblr}{
  colspec = {X[2,c]X[9]X[3,c]X[si={table-format=4},c]X[4]},
  width = \textwidth,
  row{1} = {c},
  cell{2}{1} = {r=7}{c},
  cell{2}{2} = {r=7}{},
  cell{9}{1} = {r=7}{c},
  cell{9}{2} = {r=7}{},
  cell{16}{1} = {r=4}{c},
  cell{16}{2} = {r=4}{},
  hline{1,2,20} = {-}{0.08em},
  hline{9,16} = {-}{0.05em},
}
       & \textbf{Definition}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & \textbf{Class}              & \textbf{Count} & \textbf{Example}                                    \\
\textbf{Events}       & An event refers to any occurrence, incident, action or state that takes place or holds within a specified period of time. This includes both concrete actions, such as physical movements and behaviors, as well as more abstract events, such as changes in emotional states or the passage of time or stative situations that hold during a time interval. Events have temporal relevance and can be directly related to temporal expressions. Events can be related to changes in the text and are often used to advance the plot and develop characters, but also to describe characters, objects, circumstances, places or states. & Occurrence         & 1677  & accident, fell                   \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & State              & 750   & existence, situation           \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Reporting          & 419   & announced, describes         \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Intensional Action & 97    & moved, did                          \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Perception         & 63    & discovered, receive            \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Aspectual          & 29    & started, closed                      \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Intensional State  & 22    & is forbidden, intended            \\
\textbf{Participants} & Participants refer to individuals, groups, organizations, or other entities that are actively involved in or impacted by an event or state. They are typically identified based on their relevance and significance to the situation, and may be explicitly mentioned or inferred from the context. Participants can take on a variety of roles, such as actors, agents, patients, victims, or observers, and their actions and interactions can shape the course of events.                                                                                                                                                            & Person             & 1106  & military, one man              \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Organization       & 783   & GNR, Lusa       \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Location           & 743   & Porto, the Lisbon district \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Object             & 429   & the phone, boats                      \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Other              & 274   & a house, the bodies                        \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Nature             & 137   & fire, coronavirus                  \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Facility           & 74    & hotels, the airport                    \\
\textbf{Timexs}       & Temporal expressions are linguistic elements that allow us to communicate information about time. In addition to representing specific points in time, they can also be used to classify time periods according to units such as seconds, minutes, hours, days, weeks, months, and years.                                                                                                                                                                                                                                                                                                                                               & Date               & 186   & 15/10/2020, Nov 25th                 \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Time               & 102   & early november, july                       \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Duration           & 36    & a week, four years               \\
             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Set                & 1     & daily, every two weeks                     
\end{tblr}
\end{table*}
